Embedding Probability Distributions into Low Dimensional $\ell_1$: Tree Ising Models via Truncated Metrics

Given an arbitrary set of high dimensional points in $\ell_1$, there are known negative results that preclude the possibility of always mapping them to a low dimensional $\ell_1$ space while preserving distances with small multiplicative distortion. This is in stark contrast with dimension reduction in Euclidean space ($\ell_2$) where such mappings are always possible. While the first non-trivial lower bounds for $\ell_1$ dimension reduction were established almost 20 years ago, there has been limited progress in understanding what sets of points in $\ell_1$ are conducive to a low-dimensional mapping. In this work, we study a new characterization of $\ell_1$ metrics that are conducive to dimension reduction in $\ell_1$. Our characterization focuses on metrics that are defined by the disagreement of binary variables over a probability distribution -- any $\ell_1$ metric can be represented in this form. We show that, for configurations of $n$ points in $\ell_1$ obtained from tree Ising models, we can reduce dimension to $\mathrm{polylog}(n)$ with constant distortion. In doing so, we develop technical tools for embedding truncated metrics which have been studied because of their applications in computer vision, and are objects of independent interest in metric geometry. Among other tools, we show how any $\ell_1$ metric can be truncated with $O(1)$ distortion and $O(\log(n))$ blowup in dimension.

==> unused.tex <==
    \begin{algorithm}[H]
        \caption{The snaking procedure} \label{algo:snake}
        \hspace*{\algorithmicindent} 
        \begin{flushleft}
          {\bf Input:} List of node locations $[loc]$, list of widths to snake over $[widths]$ \\
          {\bf Output:} List of embeddings for the nodes $[embedding]$ \\
        \end{flushleft}
        \begin{algorithmic}[1]
        \Procedure{Snake}{$loc, widths$}:
        \State $t \gets 0, snake \gets 0, \Delta \gets +1, n \gets len(locs)$
        \State $width \sim \mathrm{Uniform}[widths]$
        \For{$i = 1,2,\dots,n$}
            \While{$t \neq loc[i]$}
                \State $snake \gets snake + \Delta$
                \State $t \gets t+1$
                \If{$snake = width$}
                    \State $\Delta \gets -1$
                \EndIf
                \If{$snake = 0$}
                    \State $\Delta \gets +1$
                    \State $width \sim \mathrm{Uniform}[widths]$
                \EndIf
            \EndWhile
            \State $embedding[i] \gets snake$
        \EndFor
        \State {\bf return} $embedding$
        \EndProcedure
        \end{algorithmic}
    \end{algorithm}

    Consider the snaking procedure given in \Cref{algo:snake}. We set $widths = [M, 4M]$. Every invokation of \textsc{Snake}$(loc, widths)$ returns a single coordinate in the embedding of each node -- we invoke the procedure $O(\log n)$ times to obtain the final embedding.

    Let $loc'[i]=round_M(loc[i])$, where $round_M(x)$ returns the number nearest to $x$ that is a multiple of $M$ (ties broken arbitrarily), and consider instead invoking \textsc{Snake}$(loc', widths)$ to obtain $embedding'$.

    Fix a pair of nodes $x_i, x_j$ that satisfy $|loc'[i]-loc'[j]| \ge 16M$. Note that $\dcap{M}(x_i, x_j) = M$. Let $E_1$ be the event that $snake=0$ for some $t \in [\max(0, loc'[i]-8M), loc'[i]]$. Since the largest width that we snake over is $4M$, observe that $\Pr[E_1]=1$. Let $E_2$ be the event that we are at $0$ or $M$ at $t=loc'[i]$. Conditioned on $E_1$, there is at least a $\left(\frac{1}{2}\right)^4$ chance that we are at either 0 or $M$ at $t=loc'[i]$ (since the amount left to traverse is at most $8M$, we have to make a random choice of width at most 4 times, and this is the chance that we pick $width=M$ each of those times). That is, $\Pr[E_2|E_1] \ge \left(\frac{1}{2}\right)^4$.

    Now, let $E_3$ be the event that $snake=0$ for some $t \in [loc'[j]-16M, loc'[j]-8M]$. Again, we have that $\Pr[E_3]=1$, and in particular also that $\Pr[E_3|E_2, E_1]=1$. Let $E_4$ now be the event that $snake=0$ at $t=loc'[j]-4M$ or $t=loc'[j]-3M$. Conditioned on $E_1, E_2$ and $E_3$, we have that $\Pr[E_4|E_3, E_2, E_1] \ge \left(\frac{1}{2}\right)^6$ (since conditioned on $E_3$, the amount left to traverse till we get to $t=loc'[j]-4M$ is at most $12M$, and this is the chance that we pick $width=M$ each of the $\le 6$ times that we snake around till we get to either 0 or $M$ at $t=loc'[j]-4M$).

    Finally, let $E_5$ be the event that $snake=3M$ or $snake=4M$ at $t=loc'[j]$. Conditioned on all of $E_1,\dots,E_4$, we have $snake=0$ at $t=loc'[j]-4M$ or $t=loc'[j]-3M$. Then, there is a $1/2$ chance that we pick $width=4M$, which would ensure that $\Pr[E_5|E_4,E_3,E_2,E_1]\ge\frac{1}{2}$.

    Thus, we have that
    \begin{align*}
        \Pr[E_1,E_2,E_3,E_4,E_5] = \prod_{i=1}^5\Pr[E_i|E_1,\dots,E_{i-1}] \ge \left(\frac{1}{2}\right)^{11}.
    \end{align*}
    In particular, we have argued that 
    \begin{align*}
        \Pr[|embedding'[j]-embedding'[i]|\ge 2M] \ge \Pr[embedding'[i]=0 ~or~ M, embedding'[j]=3M ~or~ 4M] \ge \left(\frac{1}{2}\right)^{11}.
    \end{align*}
    Now, observe that $|loc[i]-loc'[i]|\le \frac{M}{2}$ and $|loc[j]-loc'[j]|\le \frac{M}{2}$. By the triangle inequality, we have that
    \begin{align*}
        |loc[j]-loc[i]| \ge |loc'[i]-loc'[j]| - |loc'[i]-loc[i]| - |loc'[j]-loc[j]| \ge |loc'[i]-loc'[j]|-M,
    \end{align*}
    and this same bound holds for $embedding$ and $embedding'$. Thus, we have that
    \begin{align*}
        \Pr[|embedding[j]-embedding[i]|\ge M] \ge \left(\frac{1}{2}\right)^{11}.
    \end{align*}
    Then, suppose we invoke \textsc{Snake}$(loc, widths)$ $N$ times to obtain $N$ independent copies $embedding_1,\dots,embedding_N$ for all the nodes. Let $X^{(k)}_{ij} = \Ind[|embedding_k[j]-embedding_k[i]|\ge M]$. We have from the preceding analysis that $\E[X^{(k)}_{ij}] \ge \left(\frac{1}{2}\right)^{11}.$ Furthermore, since $X^{(1)}_{ij},\dots,X^{(N)}_{ij}$ are independent, the Chernoff bound gives us that
    \begin{align*}
        \Pr\left[\sum_{k=1}^N X^{(k)}_{ij} \le 0.5N\left(\frac{1}{2}\right)^{11}\right] \le \exp\left(-N\left(\frac{1}{2}\right)^{11}\cdot(0.5)^3\right) \le \frac{1}{n^2},
    \end{align*}
    for $N = C\log n$, where $C$ is an appropriately large constant. We can now union bound over all the $< n^2$ pairs $i, j$ that satisfy $|loc'[i]-loc'[j]| \ge 16M$ to obtain that with positive probability, each one of them satisfies $\sum_{k=1}^N |embedding_k[i]-embedding_k[j]| > (0.5)^{12}MN$. Then, we simply scale each $embedding_k$ as $embedding_k \gets embedding_k/N$ to obtain that $\sum_{k=1}^N |embedding_k[i]-embedding_k[j]| > (0.5)^{12}M$. Further, note that with this scaling, $\sum_{k=1}^N |embedding_k[i]-embedding_k[j]| \le 4M$ by construction, which gives us the $O(1)$ distortion claimed in the theorem statement. 
    
    \red{say that first two coordinates are obtained by calling snake(loc, [32M]), snake(loc+16M, [32M])}

